Nonlocal control of the quantum state of light

The work is dedicated to the challenge: control and manipulation of the quantum state of a remote physical object. The goal is approached via the entanglement channel between the object and a local physical system - actuator - subjected to a quantum non-demolishing impact. Physical systems under exploration are light beams.

==> lists.tex <==
\listoffigures									% Список изображений
\addcontentsline{toc}{chapter}{\listfigurename}	% Добавляем на него ссылку в оглавление
\clearpage

\listoftables									% Список таблиц
\addcontentsline{toc}{chapter}{\listtablename}	% Добавляем на него ссылку в оглавление
\clearpage
